Finding Exogenous Variation in Data

We reconsider the classic problem of recovering exogenous variation from an endogenous regressor. Two-stage least squares recovers exogenous variation through presuming the existence of an instrumental variable. We rely instead on the assumption that the regressor is a mixture of exogenous and endogenous observations--say as the result of temporary natural experiments. With this assumption, we propose an alternative two-stage method based on nonparametrically estimating a mixture model to recover a subset of the exogenous observations. We demonstrate that our method recovers exogenous observations in simulation and can be used to find pricing experiments hidden in grocery store scanner data.

==> robustness/diff_period/all_products/accuracy.tex <==

\begin{tabular}{l|ccc|ccc}
\toprule
\multicolumn{1}{c}{\bfseries  } & \multicolumn{3}{c}{\bfseries Within Experiment Period} & \multicolumn{3}{c}{\bfseries All Data} \\
\cmidrule(l{2pt}r{2pt}){2-4} \cmidrule(l{2pt}r{2pt}){5-7}
Category & \# Stores-Weeks & \# Correct & Accuracy & \# Store-Weeks & \# Correct & Accuracy\\
\midrule
Analgesics & 448 & 261 & 0.583 & 3328 & 1179 & 0.354\\
Canned Soups & 1040 & 458 & 0.440 & 5005 & 2446 & 0.489\\
Cereals & 910 & 836 & 0.919 & 5395 & 2758 & 0.511\\
Cheese & 858 & 312 & 0.364 & 4950 & 1696 & 0.343\\
Dish Detergent & 987 & 573 & 0.581 & 4559 & 1774 & 0.389\\
Front End Candies & 840 & 659 & 0.785 & 4704 & 1832 & 0.389\\
Frozen Entrees & 1334 & 783 & 0.587 & 4756 & 2108 & 0.443\\
Snack Crackers & 944 & 875 & 0.927 & 5133 & 2575 & 0.502\\
Soft Drinks & 800 & 742 & 0.928 & 3650 & 2114 & 0.579\\
Toothpaste & 592 & 494 & 0.834 & 3441 & 1327 & 0.386\\
\bottomrule
\end{tabular}


==> robustness/diff_period/all_products/did_reg.tex <==

\begin{tabular}{lll}
\toprule
Category & Replicated & Recovered\\
\midrule
Analgesics & -1.932*** & -2.086***\\
 & (0.123) & (0.344)\\
Canned Soups & -2.729*** & -1.953***\\
 & (0.1) & (0.077)\\
Cereals & -3.031*** & -2.799***\\
 & (0.17) & (0.124)\\
Cheese & -0.314*** & -2.008***\\
 & (0.098) & (0.06)\\
Dish Detergent & -4.951*** & -4.466***\\
 & (0.147) & (0.184)\\
Front End Candies & -0.494*** & -1.177***\\
 & (0.139) & (0.36)\\
Frozen Entrees & -3.926*** & -3.636***\\
 & (0.061) & (0.112)\\
Snack Crackers & -2.882*** & -2.305***\\
 & (0.13) & (0.183)\\
Toothpaste & -1.952*** & -1.972***\\
 & (0.093) & (0.149)\\
\bottomrule
\end{tabular}


==> robustness/diff_period/all_products/did_reg_robust.tex <==

\begin{tabular}{lll}
\toprule
Category & Replicated & Recovered\\
\midrule
Analgesics & -1.925*** & NA\\
 & (0.119) & (NA)\\
Canned Soups & -2.736*** & -1.501***\\
 & (0.1) & (0.367)\\
Cereals & -3.038*** & -2.606***\\
 & (0.179) & (0.128)\\
Cheese & -0.355*** & NA\\
 & (0.09) & (NA)\\
Dish Detergent & -4.953*** & -4.749***\\
 & (0.153) & (0.406)\\
Front End Candies & -0.496*** & -0.883***\\
 & (0.144) & (0.204)\\
Frozen Entrees & -3.954*** & -3.453***\\
 & (0.06) & (0.099)\\
Snack Crackers & -2.789*** & -2.374***\\
 & (0.138) & (0.132)\\
Toothpaste & -1.975*** & -1.821***\\
 & (0.114) & (0.147)\\
\bottomrule
\end{tabular}


==> robustness/diff_period/all_products/iv.tex <==

\begin{tabular}{llll}
\toprule
Category & Replicated & Recovered & Difference\\
\midrule
Analgesics & 1.136 & -0.52*** & 1.656*\\
 & (0.832) & (0.17) & (0.849)\\
Canned Soups & -72.149 & -0.644** & -71.505\\
 & (302.753) & (0.288) & (302.753)\\
Cereals & 0.437** & -0.099 & 0.536*\\
 & (0.213) & (0.175) & (0.276)\\
Cheese & -1.186 & -0.49** & -0.696\\
 & (3.026) & (0.227) & (3.035)\\
Dish Detergent & -0.076 & -1.007*** & 0.931\\
 & (0.906) & (0.105) & (0.912)\\
Front End Candies & -0.199 & -0.167** & -0.032\\
 & (0.252) & (0.068) & (0.261)\\
Frozen Entrees & 5.972 & -2.328*** & 8.299\\
 & (29.289) & (0.787) & (29.3)\\
Snack Crackers & -81.385 & -0.613** & -80.772\\
 & (209.988) & (0.244) & (209.988)\\
Soft Drinks & -0.965** & -1.363** & 0.398\\
 & (0.477) & (0.603) & (0.769)\\
Toothpaste & -1.155*** & -0.824*** & -0.331\\
 & (0.371) & (0.171) & (0.408)\\
\bottomrule
\end{tabular}


==> robustness/diff_period/all_products/iv_robust.tex <==

\begin{tabular}{llll}
\toprule
Category & Replicated & Recovered & Difference\\
\midrule
Analgesics & 1.136 & 0.835 & 0.301\\
 & (0.832) & (0.596) & (1.023)\\
Canned Soups & -72.149 & -3.105*** & -69.044\\
 & (302.753) & (0.978) & (302.754)\\
Cereals & 0.437** & 0.187 & 0.25\\
 & (0.213) & (0.341) & (0.402)\\
Cheese & -1.186 & 0.98** & -2.166\\
 & (3.026) & (0.443) & (3.059)\\
Dish Detergent & -0.076 & -1.514*** & 1.438\\
 & (0.906) & (0.331) & (0.965)\\
Front End Candies & -0.199 & 0.392 & -0.592\\
 & (0.252) & (0.486) & (0.548)\\
Frozen Entrees & 5.972 & -2.706*** & 8.678\\
 & (29.289) & (0.571) & (29.295)\\
Snack Crackers & -81.385 & 0.037 & -81.422\\
 & (209.988) & (0.374) & (209.989)\\
Soft Drinks & -0.965** & -1.763* & 0.798\\
 & (0.477) & (0.952) & (1.065)\\
Toothpaste & -1.155*** & -1.009*** & -0.146\\
 & (0.371) & (0.26) & (0.452)\\
\bottomrule
\end{tabular}


==> robustness/diff_period/all_products/price_change.tex <==

\begin{tabular}{lrrrrrr}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{Hi-Lo} & \multicolumn{3}{c}{EDLP} \\
\cmidrule(l{2pt}r{2pt}){2-4} \cmidrule(l{2pt}r{2pt}){5-7}
 & Published & Replicated & Recovered & Published & Replicated & Recovered\\
\midrule
Analgesics & 10 & 1.847 & 4.944 & -10 & -2.250 & -3.155\\
Canned Soups & 14 & -0.032 & 4.847 & NA & NA & -5.019\\
Cereals & 10 & 4.099 & 5.395 & -10 & -5.887 & -5.542\\
Cheese & 8 & 0.425 & 2.938 & -8 & -0.375 & -3.220\\
Dish Detergent & 6 & 3.184 & 3.448 & -6 & -1.318 & -3.731\\
Front End Candies & 13 & 9.648 & 3.878 & -13 & -5.250 & -3.499\\
Frozen Entrees & 11 & 0.197 & 2.777 & -11 & 0.121 & -3.626\\
Snack Crackers & 10 & 0.042 & 2.501 & -10 & 0.086 & -2.175\\
Toothpaste & 7 & 3.743 & 2.850 & -7 & -4.470 & -3.999\\
\bottomrule
\end{tabular}


==> robustness/diff_period/all_products/price_change_robust.tex <==

\begin{tabular}{lrrrrrr}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{Hi-Lo} & \multicolumn{3}{c}{EDLP} \\
\cmidrule(l{2pt}r{2pt}){2-4} \cmidrule(l{2pt}r{2pt}){5-7}
 & Published & Replicated & Recovered & Published & Replicated & Recovered\\
\midrule
Analgesics & 10 & 1.847 & NA & -10 & -2.250 & NA\\
Canned Soups & 14 & -0.032 & 2.206 & NA & NA & -4.924\\
Cereals & 10 & 4.099 & 5.190 & -10 & -5.887 & -6.244\\
Cheese & 8 & 0.425 & NA & -8 & -0.375 & NA\\
Dish Detergent & 6 & 3.184 & 3.200 & -6 & -1.318 & -3.229\\
Front End Candies & 13 & 9.648 & 3.569 & -13 & -5.250 & -4.385\\
Frozen Entrees & 11 & 0.197 & 4.723 & -11 & 0.121 & NA\\
Snack Crackers & 10 & 0.042 & 2.424 & -10 & 0.086 & -1.979\\
Toothpaste & 7 & 3.743 & 3.855 & -7 & -4.470 & -4.097\\
\bottomrule
\end{tabular}


==> robustness/diff_period/all_products/quantity_change.tex <==

\begin{tabular}{lrrrrrr}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{Hi-Lo} & \multicolumn{3}{c}{EDLP} \\
\cmidrule(l{2pt}r{2pt}){2-4} \cmidrule(l{2pt}r{2pt}){5-7}
 & Published & Replicated & Recovered & Published & Replicated & Recovered\\
\midrule
Analgesics & 1 & 1.086 & 2.609 & 5 & 1.361 & 5.771\\
Canned Soups & -3 & -1.057 & -9.039 & NA & NA & 1.717\\
Cereals & -1 & 2.575 & -1.161 & 2 & 4.279 & -4.540\\
Cheese & -1 & 0.977 & -2.173 & 3 & 0.147 & 6.196\\
Dish Detergent & -3 & -6.163 & 1.668 & 2 & -3.863 & 10.751\\
Front End Candies & -3 & -9.809 & -12.359 & 1 & 1.106 & -15.330\\
Frozen Entrees & -8 & -0.998 & -3.215 & 10 & -0.562 & 0.080\\
Snack Crackers & -5 & -1.093 & 12.137 & -1 & -4.122 & 8.526\\
Toothpaste & -3 & -8.056 & 30.009 & 3 & 6.701 & 13.667\\
\bottomrule
\end{tabular}


==> robustness/diff_period/all_products/quantity_change_robust.tex <==

\begin{tabular}{lrrrrrr}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{Hi-Lo} & \multicolumn{3}{c}{EDLP} \\
\cmidrule(l{2pt}r{2pt}){2-4} \cmidrule(l{2pt}r{2pt}){5-7}
 & Published & Replicated & Recovered & Published & Replicated & Recovered\\
\midrule
Analgesics & 1 & 1.086 & NA & 5 & 1.361 & NA\\
Canned Soups & -3 & -1.057 & -0.727 & NA & NA & 0.778\\
Cereals & -1 & 2.575 & 3.358 & 2 & 4.279 & 1.491\\
Cheese & -1 & 0.977 & NA & 3 & 0.147 & NA\\
Dish Detergent & -3 & -6.163 & 3.112 & 2 & -3.863 & 7.859\\
Front End Candies & -3 & -9.809 & 4.582 & 1 & 1.106 & -0.918\\
Frozen Entrees & -8 & -0.998 & 10.499 & 10 & -0.562 & NA\\
Snack Crackers & -5 & -1.093 & 7.099 & -1 & -4.122 & 4.502\\
Toothpaste & -3 & -8.056 & 14.100 & 3 & 6.701 & 4.361\\
\bottomrule
\end{tabular}


==> robustness/diff_period/max_zone_week/did_reg_robust.tex <==

\begin{tabular}{lll}
\toprule
Category & Replicated & Recovered\\
\midrule
Analgesics & -1.775*** & -1.303***\\
 & (0.146) & (0.28)\\
Canned Soups & -1.135*** & -1.012***\\
 & (0.23) & (0.243)\\
Cereals & -2.69*** & -2.579***\\
 & (0.163) & (0.143)\\
Cheese & -1.42*** & -1.593***\\
 & (0.05) & (0.15)\\
Dish Detergent & -4.709*** & -4.817***\\
 & (0.16) & (0.397)\\
Front End Candies & -1.861*** & -1.249***\\
 & (0.092) & (0.172)\\
Frozen Entrees & -3.5*** & -3.454***\\
 & (0.075) & (0.095)\\
Snack Crackers & -3.08*** & -2.517***\\
 & (0.075) & (0.143)\\
Toothpaste & -5.043*** & -1.721***\\
 & (0.291) & (0.147)\\
\bottomrule
\end{tabular}


==> robustness/diff_period/max_zone_week/iv.tex <==

\begin{tabular}{llll}
\toprule
Category & Replicated & Recovered & Difference\\
\midrule
Analgesics & 0.411 & -0.391*** & 0.801\\
 & (0.573) & (0.126) & (0.586)\\
Canned Soups & 1.333 & -0.825*** & 2.159\\
 & (19.186) & (0.245) & (19.188)\\
Cereals & 0.705 & -0.124 & 0.829\\
 & (0.551) & (0.164) & (0.575)\\
Cheese & -7.298 & -0.575*** & -6.722\\
 & (5.198) & (0.201) & (5.201)\\
Dish Detergent & -0.745 & -1.104*** & 0.359\\
 & (0.899) & (0.104) & (0.905)\\
Front End Candies & 6.148*** & -0.311*** & 6.46***\\
 & (1.837) & (0.068) & (1.838)\\
Frozen Entrees & -6.574 & -2.308*** & -4.266\\
 & (5.601) & (0.765) & (5.653)\\
Snack Crackers & 0.759 & -0.611*** & 1.37\\
 & (1.176) & (0.209) & (1.194)\\
Soft Drinks & 31.814 & -1.358*** & 33.171\\
 & (48.898) & (0.429) & (48.9)\\
Toothpaste & -1.186** & -0.824*** & -0.362\\
 & (0.462) & (0.171) & (0.492)\\
\bottomrule
\end{tabular}


==> robustness/diff_period/max_zone_week/iv_robust.tex <==

\begin{tabular}{llll}
\toprule
Category & Replicated & Recovered & Difference\\
\midrule
Analgesics & 0.411 & 0.492* & -0.081\\
 & (0.573) & (0.253) & (0.626)\\
Canned Soups & 1.333 & -2.714* & 4.048\\
 & (19.186) & (1.448) & (19.241)\\
Cereals & 0.705 & 0.152 & 0.554\\
 & (0.551) & (0.328) & (0.642)\\
Cheese & -7.298 & -1.709 & -5.589\\
 & (5.198) & (1.084) & (5.309)\\
Dish Detergent & -0.745 & -1.719*** & 0.975\\
 & (0.899) & (0.257) & (0.935)\\
Front End Candies & 6.148*** & 0.183 & 5.965***\\
 & (1.837) & (0.362) & (1.872)\\
Frozen Entrees & -6.574 & -2.693*** & -3.88\\
 & (5.601) & (0.545) & (5.627)\\
Snack Crackers & 0.759 & -0.026 & 0.785\\
 & (1.176) & (0.311) & (1.216)\\
Soft Drinks & 31.814 & -1.972* & 33.785\\
 & (48.898) & (1.088) & (48.91)\\
Toothpaste & -1.186** & -1.009*** & -0.176\\
 & (0.462) & (0.26) & (0.53)\\
\bottomrule
\end{tabular}


==> robustness/diff_period/max_zone_week/price_change.tex <==

\begin{tabular}{lrrrrrr}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{Hi-Lo} & \multicolumn{3}{c}{EDLP} \\
\cmidrule(l{2pt}r{2pt}){2-4} \cmidrule(l{2pt}r{2pt}){5-7}
 & Published & Replicated & Recovered & Published & Replicated & Recovered\\
\midrule
Analgesics & 10 & 2.419 & 3.088 & -10 & -3.031 & -2.995\\
Canned Soups & 14 & -0.100 & 5.382 & NA & NA & -5.458\\
Cereals & 10 & 3.978 & 5.433 & -10 & -5.565 & -5.534\\
Cheese & 8 & -0.026 & 3.102 & -8 & -0.027 & -3.302\\
Dish Detergent & 6 & 2.963 & 3.793 & -6 & -1.112 & -4.069\\
Front End Candies & 13 & 0.811 & 5.223 & -13 & -0.693 & -4.655\\
Frozen Entrees & 11 & 0.066 & 2.834 & -11 & -0.056 & -3.699\\
Snack Crackers & 10 & 1.208 & 3.405 & -10 & -1.387 & -2.870\\
Toothpaste & 7 & 3.778 & 2.850 & -7 & -4.374 & -3.999\\
\bottomrule
\end{tabular}


==> robustness/diff_period/max_zone_week/quantity_change.tex <==

\begin{tabular}{lrrrrrr}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{Hi-Lo} & \multicolumn{3}{c}{EDLP} \\
\cmidrule(l{2pt}r{2pt}){2-4} \cmidrule(l{2pt}r{2pt}){5-7}
 & Published & Replicated & Recovered & Published & Replicated & Recovered\\
\midrule
Analgesics & 1 & -2.713 & 12.655 & 5 & -2.894 & 6.339\\
Canned Soups & -3 & -4.598 & -10.652 & NA & NA & 0.900\\
Cereals & -1 & 6.550 & -1.707 & 2 & 0.720 & -4.122\\
Cheese & -1 & -8.159 & -1.759 & 3 & -4.260 & 5.763\\
Dish Detergent & -3 & -7.548 & 2.081 & 2 & -2.333 & 11.502\\
Front End Candies & -3 & -5.004 & -11.779 & 1 & -2.841 & -13.418\\
Frozen Entrees & -8 & 3.726 & -3.561 & 10 & -0.810 & 0.003\\
Snack Crackers & -5 & 3.394 & 11.099 & -1 & -3.021 & 9.123\\
Toothpaste & -3 & -8.355 & 30.009 & 3 & 3.499 & 13.667\\
\bottomrule
\end{tabular}


==> robustness/diff_period/max_zone_week/quantity_change_robust.tex <==

\begin{tabular}{lrrrrrr}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{Hi-Lo} & \multicolumn{3}{c}{EDLP} \\
\cmidrule(l{2pt}r{2pt}){2-4} \cmidrule(l{2pt}r{2pt}){5-7}
 & Published & Replicated & Recovered & Published & Replicated & Recovered\\
\midrule
Analgesics & 1 & -2.713 & -2.454 & 5 & -2.894 & -6.568\\
Canned Soups & -3 & -4.598 & 0.098 & NA & NA & 2.194\\
Cereals & -1 & 6.550 & 3.356 & 2 & 0.720 & 1.481\\
Cheese & -1 & -8.159 & 4.146 & 3 & -4.260 & NA\\
Dish Detergent & -3 & -7.548 & 4.140 & 2 & -2.333 & 9.291\\
Front End Candies & -3 & -5.004 & 5.898 & 1 & -2.841 & 0.923\\
Frozen Entrees & -8 & 3.726 & 10.166 & 10 & -0.810 & NA\\
Snack Crackers & -5 & 3.394 & 4.854 & -1 & -3.021 & 4.763\\
Toothpaste & -3 & -8.355 & 14.100 & 3 & 3.499 & 4.361\\
\bottomrule
\end{tabular}

